DiffuMask: Synthesizing Images with Pixel-level Annotations for Semantic Segmentation Using Diffusion Models

Collecting and annotating images with pixel-wise labels is time-consuming and laborious. In contrast, synthetic data can be freely available using a generative model (e.g., DALL-E, Stable Diffusion). In this paper, we show that it is possible to automatically obtain accurate semantic masks of synthetic images generated by the Off-the-shelf Stable Diffusion model, which uses only text-image pairs during training. Our approach, called DiffuMask, exploits the potential of the cross-attention map between text and image, which is natural and seamless to extend the text-driven image synthesis to semantic mask generation. DiffuMask uses text-guided cross-attention information to localize class/word-specific regions, which are combined with practical techniques to create a novel high-resolution and class-discriminative pixel-wise mask. The methods help to reduce data collection and annotation costs obviously. Experiments demonstrate that the existing segmentation methods trained on synthetic data of DiffuMask can achieve a competitive performance over the counterpart of real data (VOC 2012, Cityscapes). For some classes (e.g., bird), DiffuMask presents promising performance, close to the stateof-the-art result of real data (within 3% mIoU gap). Moreover, in the open-vocabulary segmentation (zero-shot) setting, DiffuMask achieves a new SOTA result on Unseen class of VOC 2012. The project website can be found at https://weijiawu.github.io/DiffusionMask/.

==> CSMacrosV2.tex <==
\makeatletter
\renewcommand{\paragraph}{%
  \@startsection{paragraph}{4}%
  {\z@}{0.5ex \@plus 1ex \@minus .1ex}{-1em}%
  {\normalfont\normalsize\bfseries}%
}
\makeatother

\AtBeginDocument{%
 \abovedisplayskip=8pt plus 3pt minus 5pt
 \abovedisplayshortskip=0pt plus 3pt
 \belowdisplayskip=8pt plus 3pt minus 5pt
 \belowdisplayshortskip=5pt plus 3pt minus 4pt
}


\renewcommand{\rmdefault}{ptm}
\renewcommand{\sfdefault}{phv}

\usepackage[]{amsmath}                  %
\usepackage[]{mathtools}                %
\usepackage[]{amsthm}
\usepackage[]{amssymb,amsfonts}
\usepackage{graphicx}
\usepackage{bm}
\usepackage{bbm}

\usepackage[]{xcolor}
% \usepackage[mathscr]{eucal}

\usepackage[]{xparse}
\usepackage[]{xstring}
\usepackage{etoolbox}
\usepackage[]{xspace}
\usepackage[]{comment}

\usepackage{nicefrac}

\usepackage[margin=4pt,font=small,labelfont=bf,labelsep=endash,tableposition=top]{caption}

\usepackage{multirow}

\usepackage{url}
\def\UrlFont{\rm\small\ttfamily}

 
\makeatletter
\DeclareRobustCommand*\uell{\mathpalette\@uell\relax}
\newcommand*\@uell[2]{
  \setbox0=\hbox{$#1\ell$}
  \setbox1=\hbox{\rotatebox{10}{$#1\ell$}}
  \dimen0=\wd0 \advance\dimen0 by -\wd1 \divide\dimen0 by 2
  \mathord{\lower 0.1ex \hbox{\kern\dimen0\unhbox1\kern\dimen0}}
}
\mathcode`l="8000
\begingroup
\makeatletter
\lccode`\~=`\l
\DeclareMathSymbol{\lsb@l}{\mathalpha}{letters}{`l}
\lowercase{\gdef~{\ifnum\the\mathgroup=\m@ne  \uell  \else \lsb@l \fi}}%
\endgroup


 
               
\renewcommand{\vec}[1]{\ensuremath{\pmb{#1}}}
\newcommand{\mat}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\set}[1]{\ensuremath{\mathscr{#1}}}


\newcommand{\tensor}[1]{\ensuremath{ {\sf #1}\hspace{-0.24659cm} {\sf #1} }}




\makeatletter
\@tfor\next:=abcdefghijklmnopqrstuvwxyxz\do
{\begingroup\edef\x{\endgroup
        \noexpand\@namedef{v\next}{\noexpand\vec{\next}}%
    }\x}
\@tfor\next:=ABCDEFGHIJKLMNOPQRSTUVWXYZ\do
{\begingroup\edef\x{\endgroup
        \noexpand\@namedef{m\next}{\noexpand\mat{\next}}%
    }\x}
\@tfor\next:=ABCDEFGHIJKLMNOPQRSTUVWXYZ\do
{\begingroup\edef\x{\endgroup
        \noexpand\@namedef{s\next}{\noexpand\set{\next}}%
    }\x}
\@tfor\next:=ABCDEFGHIJKLMNOPQRSTUVWXYZ\do
{\begingroup\edef\x{\endgroup
        \noexpand\@namedef{t\next}{\noexpand\tensor{\next}}%
    }\x}
\makeatother


\def\sG{\mathcal{G}}                                %

\newcommand{\Transpose}{\ensuremath{{\!\top}} }     %
\let\T\Transpose


\newcommand{\opt}{\ensuremath{\textsc{Opt}}}

\newcommand{\norm}[1]{\ensuremath{\left\|#1 \right\|}}

\newcommand{\eyes}{\ensuremath{{\mathbf{I}}}}

\newcommand{\1}{{\mathbbm{1}}}           
                                                



\newcommand{\bcdot}{\raisebox{1pt}{\textbf{\large .}}}

\newcommand{\sdot}{\raisebox{1pt}{{.}}}



\noexpandarg
\newcommand\col[1]{%
\StrBefore{#1}{_}[\matrix]%
\StrBehind{#1}{_}[\colindex]%
{\ensuremath{{\matrix}_{ \bcdot    \mkern-1.5mu    \colindex}}}%
}

\noexpandarg
\newcommand\row[1]{%
\StrBefore{#1}{_}[\matrix]%
\StrBehind{#1}{_}[\rowindex]%
{\ensuremath{{\matrix}_{ \rowindex  \bcdot }^\T}}%
}

\noexpandarg
\DeclareDocumentCommand{\inprod}{ O{,} m }{%
\StrBefore{#2}{#1}[\leftmat]%
\StrBehind{#2}{#1}[\rightmat]%
{\ensuremath{  \left\langle \leftmat, \rightmat \right\rangle }}%
}






\renewcommand{\Pr}{\ensuremath{{\rm Pr}}}
\renewcommand{\th}{\ensuremath{^{\rm th}}}
\newcommand{\myexp}{\ensuremath{\mathbb{E}}}                    %
\newcommand{\EE}{{\mathbb{E}}}

\newcommand{\const}{\mathop{\bf   const}\nolimits}
\newcommand{\diag}{\mathop{\bf    diag}\nolimits}
\newcommand{\grad}{\mathop{\bf    grad}\nolimits}
\newcommand{\Range}{\mathop{\bf   Range}\nolimits}
\newcommand{\rank}{\mathop{\bf    rank}\nolimits}
\newcommand{\supp}{\mathop{\bf    supp}\nolimits}
\newcommand{\trace}{\mathop{\bf   trace}\nolimits}
\newcommand{\tr}{\mathop{\bf      tr}\nolimits}                 %


\makeatletter
\newcommand\@bff[1]{%
    \noexpandarg
    \IfSubStr{#1}{.}{%
      \StrBefore{#1}{.}[\firstcaption]%
      \StrBehind{#1}{.}[\secondcaption]%
      \textbf{\firstcaption.} \secondcaption}{%
      #1}%
}
\newcommand{\bcaption}[1]{\caption{\protect\@bff{#1}}}
\makeatother



\let\latexcirc=\circ
\newcommand{\ccirc}{\mathbin{\mathchoice
  {\xcirc\scriptstyle}
  {\xcirc\scriptstyle}
  {\xcirc\scriptscriptstyle}
  {\xcirc\scriptscriptstyle}
}}
\newcommand{\xcirc}[1]{\vcenter{\hbox{$#1\latexcirc$}}}
\let\circ\ccirc


\newcommand\strong[1]{\textbf{#1}}
\newcommand\foreign[1]{\emph{#1}}

\newcommand\abbrev[1]{\textsc{\lowercase{#1}}\xspace}
\let\acronym\abbrev

\newcommand{\email}[1]{\href{mailto:#1}{\nolinkurl{#1}}}
\newcommand{\code}{\texttt}
\newcommand{\command}{\texttt}


\newcommand\blue[1]{\color{blue}{{#1}}}
\newcommand\gray[1]{\color{lightgray}{{#1}}}

\let\grey\gray


\makeatletter
\newcommand\ensurecomma{\@ifnextchar,{}{\@latex@error{Don't forget the comma!}{}}}
\makeatother

\let\eg=\relax
\let\ie=\relax
\let\cf=\relax
\let\etc=\relax
\let\etal=\relax

\newcommand\eg{\foreign{e.g.}\ensurecomma}
\newcommand\ie{\foreign{i.e.}\ensurecomma}
\newcommand\cf{\foreign{cf.\xspace}}

\makeatletter
\newcommand\ensuresingleperiod{\@ifnextchar.{}{.\xspace}}
\makeatother

\newcommand\etc{\foreign{etc}\ensuresingleperiod}
\newcommand\etal{\foreign{et al}\ensuresingleperiod}


\usepackage{expl3,xparse}               %
\ExplSyntaxOn
\cs_new_eq:Nc \emph_old:n { emph~ }     %
\cs_new_eq:NN \emph_braces:n \textup    %
\cs_new:Npn \emph_new:n #1 {
  \tl_set:Nn \l_emph_tl {#1}
  \tl_replace_all:Nnn \l_emph_tl {(}{\emph_braces:n{(}}
  \tl_replace_all:Nnn \l_emph_tl {)}{\emph_braces:n{)}}
  \tl_replace_all:Nnn \l_emph_tl {[}{\emph_braces:n{[}}
  \tl_replace_all:Nnn \l_emph_tl {]}{\emph_braces:n{]}}
  \exp_args:NV \emph_old:n \l_emph_tl
}
\RenewDocumentCommand {\emph} {sm} {
  \IfBooleanTF {#1} {\emph_old:n {#2}} {\emph_new:n {#2}}
}
\ExplSyntaxOff


==> tables/COCO2017.tex <==
\tablestyle{4pt}{1.2}\scriptsize\begin{tabular}{l|l |l | ccccccc|ccccccc | c}
  & & & \multicolumn{14}{c|}{Semantic Segmentation~(IoU) for Selected Class/\%} & \\
  & & & \multicolumn{7}{c|}{Top 7} & \multicolumn{7}{c|}{Bottom 7} & \\
Train Set & Number & Backbone & aeroplane & bird & boat & bus & car & cat & chair & cow & dog & horse & chair & cow & dog & horse & mIoU \\
  \shline
  \multicolumn{18}{l}{\textbf{\textit{Train with Real Data}}}
  % \textbf{\textit{Train with Real Data}} & &  &  &  &  &   &  &  & &  &   &  &  &  &  &  &   \\
  \\
  \multirow{2}{*}{COCO 2017}
  & 118.2k & R50 &  - & - & - &  - & - & - & - & - &  - & - & - & - &  - & - & 61.7  \\
  & 118.2k & Swin-B & - & - & - &  - & - & - & - & - &  - & - & - & - &  - & - & -   \\
   \hline
   \multicolumn{18}{l}{\textbf{\textit{Train with Pure Synthetic Data}}}\\
   % \textit{Synthetic Data} & &  &  &  &  &   &  &  & &  &   &  &  &  &  &  &   \\
  \multirow{2}{*}{\textbf{\diffmask}}
  & - & R50\phantom{$^{\text{\textdagger}}$} & - & - & - &  - & - & - & - & - &  - & - & - & - &  - & - & -  \\
  & - & Swin-B\phantom{$^{\text{\textdagger}}$} & - & - & - & - & - &  - & - & - & - & - &  -  & - &  - & - & - \\
   \hline
  \multirow{2}{*}{COCO 2017, \textbf{\diffmask}}
  & - & R50\phantom{$^{\text{\textdagger}}$} & - & - & - & - &  - & - & - & - &  - & - & -  & - &  - & - & -\\
  & - & Swin-B\phantom{$^{\text{\textdagger}}$} & - & - & - & - & - & - & - & - &  - & - & - & - &  - & - & - \\
  
  \end{tabular}

==> tables/COCO_all_class.tex <==
\tablestyle{4pt}{1.2}\scriptsize\begin{tabular}{l|cccccccccc}
  &  \multicolumn{10}{c}{1-10 classes}  \\
  % & & & \multicolumn{7}{c|}{Top 7} & \multicolumn{7}{c|}{Bottom 7} & \\
 Train Set & person & bicycle & car & motorcycle & airplane & bus & train & truck & boat & traffic light  \\
  \shline
  % \multicolumn{18}{l}{\textbf{\textit{Train with Real Data}}}
  % \textbf{\textit{Train with Real Data}} & &  &  &  &  &   &  &  & &  &   &  &  &  &  &  &   \\
  \\
  COCO 2017
  & 82.9 & 65.7 &  56.9 & 78.3 & 73.2 &  79.9 & 80.8 & 56.0 & 57.4 & 62.4  \\
  \Ours
  & 73.4 & - &  - & - & - &  - & - & - & - & -  \\
  \hline
  &  \multicolumn{10}{c}{11-20 classes}  \\
  & fire hydrant & stop sign & parking meter & bench & bird & cat & dog & horse & sheep & cow\\
  COCO 2017
  & 88.5 & 90.7 &  68.0 & 50.0 & 71.5 &  87.7 & 77.9 & 79.1 & 79.6 & 74.2  \\
  \Ours
  & - & - &  - & - & - &  - & - & - & - & -  \\
  \hline
  &  \multicolumn{10}{c}{21-30 classes}  \\
  & elephant & bear & zebra & giraffe & backpack & umbrella & handbag & tie & suitcase & frisbee \\
  COCO 2017
  & 90.6 & 89.3 &  91.3 & 85.8 & 37.3 &  72.5 & 31.3 & 63.2 & 75.2 & 44.6  \\
  \Ours
  & - & - &  - & - & - &  - & - & - & - & -  \\
  \hline
  &  \multicolumn{10}{c}{31-40 classes}  \\
  & skis & snowboard & sports ball &kite & baseball bat & baseball glove & skateboard & surfboard & tennis racket&bottle \\
  COCO 2017
  & 32.4 & 38.9 &  43.2 & 56.9 & 22.4 &  54.8 & 65.3 & 67.7 & 70.6 & 55.5  \\
  \Ours
  & - & - &  - & - & - &  - & - & - & - & -  \\
  \hline
  &  \multicolumn{10}{c}{41-50 classes}  \\
  & wine glass & cup & fork &knife & spoon & bowl & banana & apple & sandwich &orange \\
  COCO 2017
  & 66.7 & 59.2 &  46.1 & 40.5 & 36.6 &  49.3 & 79.5 & 51.1 & 55.7 & 71.8  \\
  \Ours
  & - & - &  - & - & - &  - & - & - & - & -  \\
  \hline
  &  \multicolumn{10}{c}{51-60 classes}  \\
  & broccoli & carrot & hot dog & pizza & donut & cake & chair & couch & potted plant & bed \\
  COCO 2017
  & 63.1 & 51.1 &  50.9 & 79.5 & 63.9 &  59.1 & 42.3 & 54.8 & 29.8 & 62.8  \\
  \Ours
  & - & - &  - & - & - &  - & - & - & - & -  \\
  &  \multicolumn{10}{c}{61-70 classes}  \\
  & dining table & toilet & tv & laptop & mouse & remote & keyboard & cell phone & microwave & oven \\
  COCO 2017
  & 43.8 & 76.8 &  65.7 & 67.7 & 53.7 &  46.2 & 60.3 & 67.0 & 48.1 & 55.4  \\
  \Ours
  & - & - &  - & - & - &  - & - & - & - & -  \\
  &  \multicolumn{10}{c}{71-80 classes}  \\
  & toaster & sink & refrigerator & book & clock & vase & scissors & teddy bear & hair drier & toothbrush \\
  COCO 2017
  & 52.8 & 62.1 &  75.9 & 46.9 & 61.6 & 51.8 & 78.6 & 79.1 & 21.7 & 28.3 \\
  \Ours
  & - & - &  - & - & - &  - & - & - & - & -  \\
  
  \end{tabular}

==> tables/VOC_all_class.tex <==
\tablestyle{4pt}{1.2}\scriptsize\begin{tabular}{l|cccccccccc}
  &  \multicolumn{10}{c}{1-10 classes}  \\
  % & & & \multicolumn{7}{c|}{Top 7} & \multicolumn{7}{c|}{Bottom 7} & \\
 Train Set & aeroplane & bicycle & car & motorcycle & airplane & bus & train & truck & boat & traffic light  \\
  \shline
  % \multicolumn{18}{l}{\textbf{\textit{Train with Real Data}}}
  % \textbf{\textit{Train with Real Data}} & &  &  &  &  &   &  &  & &  &   &  &  &  &  &  &   \\
  \\
  COCO 2017
  & 82.9 & 65.7 &  56.9 & 78.3 & 73.2 &  79.9 & 80.8 & 56.0 & 57.4 & 62.4  \\
  \Ours
  & 73.4 & - &  - & - & - &  - & - & - & - & -  \\
  \hline
  &  \multicolumn{10}{c}{11-20 classes}  \\
  & fire hydrant & stop sign & parking meter & bench & bird & cat & dog & horse & sheep & cow\\
  COCO 2017
  & 88.5 & 90.7 &  68.0 & 50.0 & 71.5 &  87.7 & 77.9 & 79.1 & 79.6 & 74.2  \\
  \Ours
  & - & - &  - & - & - &  - & - & - & - & -  \\
  \hline
  &  \multicolumn{10}{c}{21-30 classes}  \\
  & elephant & bear & zebra & giraffe & backpack & umbrella & handbag & tie & suitcase & frisbee \\
  COCO 2017
  & 90.6 & 89.3 &  91.3 & 85.8 & 37.3 &  72.5 & 31.3 & 63.2 & 75.2 & 44.6  \\
  \Ours
  & - & - &  - & - & - &  - & - & - & - & -  \\
  \hline
  &  \multicolumn{10}{c}{31-40 classes}  \\
  & skis & snowboard & sports ball &kite & baseball bat & baseball glove & skateboard & surfboard & tennis racket&bottle \\
  COCO 2017
  & 32.4 & 38.9 &  43.2 & 56.9 & 22.4 &  54.8 & 65.3 & 67.7 & 70.6 & 55.5  \\
  \Ours
  & - & - &  - & - & - &  - & - & - & - & -  \\
  \hline
  &  \multicolumn{10}{c}{41-50 classes}  \\
  & wine glass & cup & fork &knife & spoon & bowl & banana & apple & sandwich &orange \\
  COCO 2017
  & 66.7 & 59.2 &  46.1 & 40.5 & 36.6 &  49.3 & 79.5 & 51.1 & 55.7 & 71.8  \\
  \Ours
  & - & - &  - & - & - &  - & - & - & - & -  \\
  \hline
  &  \multicolumn{10}{c}{51-60 classes}  \\
  & broccoli & carrot & hot dog & pizza & donut & cake & chair & couch & potted plant & bed \\
  COCO 2017
  & 63.1 & 51.1 &  50.9 & 79.5 & 63.9 &  59.1 & 42.3 & 54.8 & 29.8 & 62.8  \\
  \Ours
  & - & - &  - & - & - &  - & - & - & - & -  \\
  &  \multicolumn{10}{c}{61-70 classes}  \\
  & dining table & toilet & tv & laptop & mouse & remote & keyboard & cell phone & microwave & oven \\
  COCO 2017
  & 43.8 & 76.8 &  65.7 & 67.7 & 53.7 &  46.2 & 60.3 & 67.0 & 48.1 & 55.4  \\
  \Ours
  & - & - &  - & - & - &  - & - & - & - & -  \\
  &  \multicolumn{10}{c}{71-80 classes}  \\
  & toaster & sink & refrigerator & book & clock & vase & scissors & teddy bear & hair drier & toothbrush \\
  COCO 2017
  & 52.8 & 62.1 &  75.9 & 46.9 & 61.6 & 51.8 & 78.6 & 79.1 & 21.7 & 28.3 \\
  \Ours
  & - & - &  - & - & - &  - & - & - & - & -  \\
  
  \end{tabular}

==> tables/augmentation.tex <==
\tablestyle{4pt}{1.2}\scriptsize\begin{tabular}{c|cc|c}
  Method & Bird & Dog  &\textit{mIoU} \\
  \shline
  -  &  & & \\
  Splicing &  & & \\
  Splicing\&Blur\&Occlusion &  &  & \\
  Splicing\&Blur\&Occlusion\&PT &  &  & 
  
  \end{tabular}



==> tables/cityscapes.tex <==
\tablestyle{4pt}{1.2}\scriptsize\begin{tabular}{l|l |l || cc||cc|c||cccccc|c || c}
    & & & \multicolumn{2}{c||}{Stuff/\%} & \multicolumn{10}{c||}{Things/\%} &\\
  & & & &&\multicolumn{3}{c||}{Human/\%} & \multicolumn{7}{c||}{Vehicle/\%} &\\
Train Set & Number & Backbone & traffic light & vegetation & person & rider & mIoU & car & truck & bus  & train  & motorcycle & bicycle  & mIoU & mIoU \\
  \shline
  \multicolumn{16}{l}{\textit{Train with \textbf{Real} Data}}\\
  % \textit{Real Data} & & & & &  &  &  &   &  &  & &  &   &    \\
  \multirow{2}{*}{Cityscapes}
  & 3.0k & R50 &  66.6 & 92.6 & 83.0 & 59.2 & & 94.5 & 64.5 & 91.9 & 81.1 &  67.6 & 78.1 & &77.5  \\
  & 3.0k & Swin-B & - & - & - &  - & - & - & - & - &  - & - & - & - & -  \\
   \hline
   \multicolumn{16}{l}{\textit{Train with Pure \textbf{Synthetic} Data}}\\
   % \textit{Synthetic Data} & &  &  &    &   &  &  & &  &   &  &  & & &   \\
  \multirow{2}{*}{\textbf{\diffmask}}
  & - & R50\phantom{$^{\text{\textdagger}}$} &  &  & 56.6 & & & 82.5 & 10.6 & 50.2  & - & & 53.0 &  & - \\
  & - & Swin-B\phantom{$^{\text{\textdagger}}$} & - & - & - & - & - & &  - & - & - & -  &  - & -  & \\
   \hline
  \multirow{2}{*}{Cityscapes, \textbf{\diffmask}}
  & - & R50\phantom{$^{\text{\textdagger}}$} & - & - & - & - &  - & - & & & - & - &  -  & - & - \\
  & - & Swin-B\phantom{$^{\text{\textdagger}}$} & - & - & - & - & - & - & & &- & - &  - & - & - \\
  
  \end{tabular}


%   classes          IoU      nIoU
% --------------------------------
% road          : 0.984      nan
% sidewalk      : 0.868      nan
% building      : 0.927      nan
% wall          : 0.500      nan
% fence         : 0.607      nan
% pole          : 0.691      nan
% traffic light : 0.660      nan
% traffic sign  : 0.768      nan
% vegetation    : 0.926      nan
% terrain       : 0.650      nan
% sky           : 0.949      nan
% person        : 0.830    0.652
% rider         : 0.592    0.348
% car           : 0.945    0.875
% truck         : 0.645    0.334
% bus           : 0.919    0.641
% train         : 0.811    0.541
% motorcycle    : 0.676    0.352
% bicycle       : 0.781    0.566
% --------------------------------
% Score Average : 0.775    0.539

==> tables/feature.tex <==
\tablestyle{4pt}{1.2}\scriptsize\begin{tabular}{l|cc|c}
  Attention Map $\mathcal{A}$ & Bird & Dog  &\textit{mIoU} \\
  \shline
   $8\times8$ & 40.5   & 46.0 &  43.3 \\ $16\times16$ & 58.8   & 69.9 &  64.4\\
   $32\times32$ & 86.2   & 82.3 &  84.3\\
   $64\times64$ & 45.2   & 41.1 &  43.2\\
   $16\times16$,$32\times32$,$32\times32$ & 89.9   & 84.2 &  87.1\\
   Average & 92.9   & 86.0 &  89.5

  \end{tabular}



==> tables/rebu_distored.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\def\x{{$\scriptsize \times$}}
\footnotesize 
\setlength{\tabcolsep}{2pt}
\begin{tabular}{c|c|c|c}
% \whline


 &  & Random Dilation and Erosion &\\
Training Set & Normal & kernel: $3\times3$, $5\times5$, $8\times8$, $12\times12$& Improv.
\\\hline
\hline

VOC 2012~(Ground Truth) & 83.4 & 82.2 & -$1.2\%$\\
DiffuMask~(Generated Mask) &  70.6  & 69.3 & -$1.3\%$
% \\
% VOC 2012+DiffuMask  & 84.9 &85.0 & 85.0 & 84.7 & 84.6& 84.7 






\end{tabular}


% VOC 2012~(Ground Truth) & 83.4 & 83.1 & 83.1 & 83.0 &82.9 & 83.3\\
% DiffuMask~(Generated Mask) &  70.6 & 70.1 & 70.0 & 70.3 & 70.4 & 70.3
% \\
% VOC 2012+DiffuMask  & 84.9 &85.0 & 85.0 & 84.7 & 84.6& 84.7 
